Mapping of Parent Hamiltonians: from Abelian and non-Abelian Quantum Hall States to Exact Models of Critical Spin Chains

This monograph introduces an exact model for a critical spin chain with arbitrary spin S, which includes the Haldane--Shastry model as the special case S=1/2. While spinons in the Haldane--Shastry model obey abelian half-fermi statistics, the spinons in the general model introduced here obey non-abelian statistics. This manifests itself through topological choices for the fractional momentum spacings. The general model is derived by mapping exact models of quantized Hall states onto spin chains. The book begins with pedagogical review of all the relevant models including the non-abelian statistics in the Pfaffian Hall state, and is understandable to every student with a graduate course in quantum mechanics.

==> references.tex <==
\begin{thebibliography}{100}

\bibitem{affleck90proc}
I.~Affleck, \emph{Field theory methods and quantum critical phenomena}, in
  E.~Br\'ezin and J.~Zinn-Justin, eds., \emph{Fields, strings and critical
  phenomena}, volume XLIX of \emph{Les {H}ouches lectures} (Elsevier,
  Amsterdam, 1990).

\bibitem{affleck-87prl799}
I.~Affleck, T.~Kennedy, E.~H. Lieb, and H.~Tasaki, \emph{Rigorous results on
  valence-bond ground states in antiferromagnets}, Phys. Rev. Lett.
  \textbf{59},  799 (1987).

\bibitem{affleck-88cmp477}
---, \emph{Valence bond ground states in isotropic quantum antiferromagnets},
  Commun. Math. Phys. \textbf{115},  477 (1988).

\bibitem{anderson66rmp298}
P.~Anderson, \emph{Considerations on the {F}low of {S}uperfluid {H}elium}, Rev.
  of Mod. Phys. \textbf{38},  298 (1966).

\bibitem{anderson87s1196}
P.~W. Anderson, \emph{The resonating valence bond state in
  $\text{La}_2\text{CuO}_4$ and superconductivity}, Science \textbf{235},  1196
  (1987).

\bibitem{arovas-84prl722}
D.~Arovas, J.~R. Schrieffer, and F.~Wilczek, \emph{Fractional statistics and
  the quantum {H}all effect}, Phys. Rev. Lett. \textbf{53},  722 (1984).

\bibitem{Arovas86}
D.~P. Arovas, \emph{Fear and loathing in the lowest {Landau} level}, Ph.D.
  thesis, University of California, Santa Barbara (1986).

\bibitem{arovas-88prl531}
D.~P. Arovas, A.~Auerbach, and F.~D.~M. Haldane, \emph{Extended {H}eisenberg
  models of antiferromagnetism: Analogies to the fractional quantum {Hall}
  effect}, Phys. Rev. Lett. \textbf{60},  531 (1988).

\bibitem{arovas-85npb117}
D.~P. Arovas, R.~Schrieffer, F.~Wilczek, and A.~Zee, \emph{Statistical
  mechanics of anyons}, Nucl. Phys. B \textbf{251},  117  (1985).

\bibitem{Auerbach94}
A.~Auerbach, \emph{Interacting electrons and quantum magnetism} (Springer, New
  York, 1994).

\bibitem{bardeen-57pr162}
J.~Bardeen, L.~N. Cooper, and J.~R. Schrieffer, \emph{Microscopic theory of
  superconductivity}, Phys. Rev. \textbf{106},  162 (1957).

\bibitem{baym69}
G.~Baym, \emph{Lectures on Quantum Mechanics} (Benjamin/Addison Wesley, New
  York, 1969).

\bibitem{bernevig-01prb024425}
B.~A. Bernevig, D.~Giuliano, and R.~B. Laughlin, \emph{Coordinate
  representation of the two-spinon wave function and spinon interaction in the
  {Haldane--Shastry} model}, Phys. Rev.~B \textbf{64},  024425 (2001).

\bibitem{bernevig-01prl3392}
---, \emph{Spinon attraction in spin-1/2 antiferromagnetic chains}, Phys. Rev.
  Lett. \textbf{86},  3392 (2001).

\bibitem{bernevig-08prl246802}
B.~A. Bernevig and F.~D.~M. Haldane, \emph{Model fractional quantum {{Hall}}
  states and {Jack} polynomials}, Phys. Rev. Lett. \textbf{100},  246802
  (2008).

\bibitem{berry84prsla45}
M.~V. Berry, \emph{Quantal phase factors accompanying adiabatic changes}, Proc.
  R. Soc. Lond. A \textbf{392},  45–57 (1984).

\bibitem{bishara-09prb155303}
W.~Bishara, P.~Bonderson, C.~Nayak, K.~Shtengel, and J.~K. Slingerland,
  \emph{Interferometric signature of non-{Abelian} anyons}, Phys. Rev. B
  \textbf{80},  155303 (2009).

\bibitem{ChakrabortyPietilainen95}
T.~Chakraborty and P.~Pietil{\"a}inen, \emph{The Fractional Quantum Hall
  Effect} (Springer, New York, 1995), second edition.

\bibitem{chang-84prl997}
A.~M. Chang, P.~Berglund, D.~C. Tsui, H.~L. Stormer, and J.~C.~M. Hwang,
  \emph{Higher-order states in the multiple-series, fractional, quantum {Hall}
  effect}, Phys. Rev. Lett. \textbf{53},  997 (1984).

\bibitem{ChariPressley98}
V.~Chari and A.~Pressley, \emph{A {G}uide to {Q}uantum {G}roups} (Cambridge
  University Press, Cambridge, 1998).

\bibitem{clark-86ss141}
R.~Clark, R.~Nicholas, A.~Usher, C.~Foxon, and J.~Harris, \emph{Odd and even
  fractionally quantized states in {G}a{A}s-{G}a{A}l{A}s heterojunctions},
  Surf. Sci. \textbf{170},  141  (1986).

\bibitem{dasSarma-05prl166802}
S.~Das~Sarma, M.~Freedman, and C.~Nayak, \emph{Topologically-protected qubits
  from a possible non-{Abelian} fractional quantum {Hall} state}, Phys. Rev.
  Lett. \textbf{94},  166802 (2005).

\bibitem{dirac31prsla60}
P.~A.~M. Dirac, \emph{Quantised singularities in the electromagnetic field},
  Proc. Roy. Soc. London, Ser. A \textbf{133},  60 (1931).

\bibitem{dolev-08n829}
M.~Dolev, M.~Heiblum, V.~Umansky, A.~Stern, and D.~Mahalu, \emph{Observation of
  a quarter of an electron charge at the $\nu=5/2$ quantum {Hall} state},
  Nature \textbf{452},  829 (2008).

\bibitem{Drinfeld85smd254}
V.~G. Drinfel'd, \emph{Hopf algebras and the quantum {Y}ang--{B}axter
  equation}, Sov. Math. Dokl. \textbf{31},  254 (1985).

\bibitem{DysonQuotedinSchrieffer64}
F.~Dyson, quoted in \cite{Schrieffer64}, page 42.

\bibitem{eskes-88prl1415}
H.~Eskes and G.~A. Sawatzky, \emph{Tendency towards local spin compensation of
  holes in the high-${T}_{\rm c}$ copper compounds}, Phys. Rev. Lett.
  \textbf{61},  1415 (1988).

\bibitem{essler95prb13357}
F.~H.~L. E{\ss}ler, \emph{A note on dressed {S}-matrices in models with
  long-range interactions}, Phys. Rev.~B \textbf{51},  13357 (1995).

\bibitem{fano-86prb2670}
G.~Fano, F.~Ortolani, and E.~Colombo, \emph{Configuration-interaction
  calculations on the fractional quantum {Hall} effect}, Phys. Rev. B
  \textbf{34},  2670 (1986).

\bibitem{Fradkin91}
E.~Fradkin, \emph{Field Theories of Condensed Matter Systems}, number~82 in
  Frontiers in Physics (Addison Wesley, Redwood City, 1991).

\bibitem{fradkin-98npb704}
E.~Fradkin, C.~Nayak, A.~Tsvelik, and F.~Wilczek, \emph{A chern-simons
  effective field theory for the {Pfaffian} quantum {Hall} state}, Nucl. Phys.
  B \textbf{516},  704 (1998).

\bibitem{freedman-02cmp587}
M.~H. Freedman, A.~Kitaev, and Z.~Wang, \emph{Simulation of topological field
  theories by quantum computer}, Comm. Math. Phys. \textbf{227},  587 (2002).

\bibitem{frobenius-1882ram53}
G.~Frobenius, \emph{Ueber die elliptischen {Funktionen} zweiter {Art}}, J.
  Reine Angew. Math. \textbf{93},  53 (1882).

\bibitem{froehlich-88lmp347}
J.~Fr{\"o}hlich and P.-A. Marchetti, \emph{Quantum field theory of anyons},
  Lett. Math. Phys. \textbf{16},  347 (1988).

\bibitem{gaudin73jpp511}
M.~Gaudin, \emph{Gaz coulombien discret {\`a} une dimension}, J. Phys. (Paris)
  \textbf{34},  511 (1973).

\bibitem{gebhardt-87prl1472}
F.~Gebhard and D.~Vollhardt, \emph{Correlation functions for {Hubbard}-type
  models: The exact results for the {Gutzwiller} wave function in one
  dimension}, Phys. Rev. Lett. \textbf{59},  1472 (1987).

\bibitem{deGennes66}
P.~G. de~Gennes, \emph{Superconductivity of {M}etals and {A}lloys}
  (Benjamin/Addison Wesley, New York, 1966).

\bibitem{girvin-83prb4506}
S.~M. Girvin and T.~Jach, \emph{Interacting electrons in two-dimensional
  {Landau} levels: Results for small clusters}, Phys. Rev. B \textbf{28},  4506
  (1983).

\bibitem{goldhaber-89mpla21}
A.~S. Goldhaber, R.~MacKenzie, and F.~Wilczek, \emph{Field corrections to
  induced statistics}, Mod. Phys. Lett. A \textbf{4},  21 (1989).

\bibitem{gottfried66}
K.~Gottfried, \emph{Quantum mechanics}, volume I: Fundamentals
  (Benjamin/Addison Wesley, New York, 1966).

\bibitem{greiter93baps137}
M.~Greiter, \emph{Root configurations and many body interactions for
  fractionally quantized {Hall} states}, Bull. Am. Phys. Soc. \textbf{38},  137
  (1993).

\bibitem{greiter94plb48}
---, \emph{Microscopic formulation of the hierarchy of quantized {Hall}
  states}, Phys. Lett. B \textbf{336},  48 (1994).

\bibitem{greiter97pe1}
---, \emph{Quantum {Hall} quarks}, Physica E \textbf{1},  1  (1997).

\bibitem{greiter02jltp1029}
---, \emph{{S=1} spin liquids: {B}roken discrete symmetries restored}, J.~Low
  Temp. Phys. \textbf{126},  1029 (2002).

\bibitem{greiter05ap217}
---, \emph{Is electromagnetic gauge invariance spontaneously violated in
  superconductors?}, Ann. Phys. \textbf{319},  217 (2005).

\bibitem{greiter09prb064409}
---, \emph{Statistical phases and momentum spacings for one-dimesional anyons},
  Phys. Rev. B \textbf{79},  064409 (2009).

\bibitem{greiter10np5}
---, \emph{Quantum many-body physics: Confinement in a quantum magnet}, Nat.\
  Phys.\ \textbf{6},  5 (2010).

\bibitem{greiter11prb115129}
---, \emph{{Landau} level quantization on the sphere}, Phys. Rev. B
  \textbf{83},  115129 (2011).

\bibitem{greiter-07prb184441}
M.~Greiter and S.~Rachel, \emph{Valence bond solids for {SU($n$)} spin chains:
  Exact models, spinon confinement, and the {H}aldane gap}, Phys. Rev. B
  \textbf{75},  184441 (2007).

\bibitem{greiter-05prb224424}
M.~Greiter and D.~Schuricht, \emph{No attraction between spinons in the
  {H}aldane--{S}hastry model}, Phys. Rev.~B \textbf{71},  224424 (2005).

\bibitem{greiter-06prl059701}
---, \emph{Comment on {"Spinon Attraction in Spin-1/2 Antiferromagnetic
  Chains"}}, Phys. Rev. Lett. \textbf{96},  059701 (2006).

\bibitem{greiter-07prl237202}
---, \emph{Many-spinon states and the secret significance of {Young} tableaux},
  Phys. Rev. Lett. \textbf{98},  237202 (2007).

\bibitem{greiter-09prl207203}
M.~Greiter and R.~Thomale, \emph{Non-{Abelian} statistics in a quantum
  antiferromagnet}, Phys. Rev. Lett. \textbf{102},  207203 (2009).

\bibitem{greiter-91prl3205}
M.~Greiter, X.~G. Wen, and F.~Wilczek, \emph{Paired {Hall} state at half
  filling}, Phys. Rev. Lett. \textbf{66},  3205 (1991).

\bibitem{greiter-92npb567}
---, \emph{Paired {Hall} states}, Nucl. Phys. B \textbf{374},  567 (1992).

\bibitem{greiter-90mplb1063}
M.~Greiter and F.~Wilczek, \emph{Heuristic principle for quantized {Hall}
  states}, Mod. Phys. Lett. B \textbf{4},  1063 (1990).

\bibitem{greiter-92npb577}
---, \emph{Exact solutions and the adiabatic heuristic for quantum {Hall}
  states}, Nucl. Phys. B \textbf{370},  577 (1992).

\bibitem{gros-87prb381}
C.~Gros, R.~Joynt, and T.~M. Rice, \emph{Antiferromagnetic correlations in
  almost-localized fermi liquids}, Phys. Rev. B \textbf{36},  381 (1987).

\bibitem{gutzwiller63prl159}
M.~C. Gutzwiller, \emph{Effect of correlation on the ferromagnetism of
  transition metals}, Phys. Rev. Lett. \textbf{10},  159 (1963).

\bibitem{ha-93prb12459}
Z.~N.~C. Ha and F.~D.~M. Haldane, \emph{Squeezed strings and {Y}angian symmetry
  of the {H}eisenberg chain with long-range interaction}, Phys. Rev.~B
  \textbf{47},  12459 (1993).

\bibitem{ha-94prl2887}
---, \emph{Elementary excitations of one-dimensional {$t$}-{$J$} model with
  inverse-square exchange}, Phys. Rev. Lett. \textbf{73},  2887 (1994).
  \emph{ibid.} \textbf{74}, E3501 (1995).

\bibitem{haldane83pl464}
F.~D.~M. Haldane, \emph{Contiuum dynamics of the {1-D} {Heisenberg}
  antiferromagnet: {I}dentification with the {O(3)} nonlinear sigma model},
  Phys. Lett. \textbf{93 A},  464 (1983).

\bibitem{haldane83prl605}
---, \emph{Fractional quantization of the {Hall} effect: {A} hierarchy of
  incompressible quantum fluid states}, Phys. Rev. Lett. \textbf{51},  605
  (1983).

\bibitem{haldane83prl1153}
---, \emph{Nonlinear field theory of large-spin {Heisenberg} antiferromagnets:
  {S}emiclassically quantized solitons of the one-dimensional easy-axis
  {N\'{e}el} state}, Phys. Rev. Lett. \textbf{50},  1153 (1983).

\bibitem{haldane88prl635}
---, \emph{Exact {Jastrow--Gutzwiller} resonant-valence-bond ground state of
  the spin-$\frac{1}{2}$ antiferromagnetic {Heisenberg} chain with $1/r^2$
  exchange}, Phys. Rev. Lett. \textbf{60},  635 (1988).

\bibitem{haldane91prl937}
---, \emph{"{F}ractional statistics"\ in arbitrary dimensions: {A}
  generalization of the {Pauli} principle}, Phys. Rev. Lett. \textbf{67},  937
  (1991).

\bibitem{haldane91prl1529}
---, \emph{"{S}pinon gas"\ description of the {$S=\tfrac{1}{2}$} {H}eisenberg
  chain with inverse-square exchange: {E}xact spectrum and thermodynamics},
  Phys. Rev. Lett. \textbf{66},  1529 (1991).

\bibitem{haldane94proc}
---, \emph{Physics of the ideal semion gas: {S}pinons and quantum symmetries of
  the integrable {Haldane--Shastry} spin chain}, in A.~Okiji and N.~Kawakami,
  eds., \emph{Correlation Effects in Low-Dimensional Electron Systems}
  (Springer, Berlin, 1994).

\bibitem{haldane-92prl2021}
F.~D.~M. Haldane, Z.~N.~C. Ha, J.~C. Talstra, D.~Bernard, and V.~Pasquier,
  \emph{Yangian symmetry of integrable quantum chains with long-range
  interactions and a new description of states in conformal field theory},
  Phys. Rev. Lett. \textbf{69},  2021 (1992).

\bibitem{haldane-85prb2529}
F.~D.~M. Haldane and E.~H. Rezayi, \emph{Periodic {Laughlin--Jastrow} wave
  functions for the fractional quantized {Hall} effect}, Phys. Rev. B
  \textbf{31},  2529 (1985).

\bibitem{halperin83hpa75}
B.~I. Halperin, \emph{Theory of the quantized {Hall} conductance}, Helvetica
  Physica Acta \textbf{56},  75 (1983).

\bibitem{halperin84prl1583}
---, \emph{Statistics of quasiparticles and the hierarchy of fractional
  quantized {Hall} states}, Phys. Rev. Lett. \textbf{52},  1583 (1984).
  \emph{ibid.} \textbf{52}, E2390 (1984).

\bibitem{Hamermesh62}
M.~Hamermesh, \emph{Group Theory and its Application to Physical Problems}
  (Addison--Wesley, Reading, Mass., 1962).

\bibitem{inozemtsev90jsp1143}
V.~I. Inozemtsev, \emph{On the connection between the one-dimensional {$S=1/2$}
  {Heisenberg} chain and {Haldane}--{Shastry} model}, J. Stat. Phys.
  \textbf{59},  1143 (1990).

\bibitem{InuiTanabeOnodera96}
T.~Inui, Y.~Tanabe, and Y.~Onodera, \emph{Group Theory and Its Applications in
  Physics} (Springer, Berlin, 1996).

\bibitem{ivanov01prl268}
D.~A. Ivanov, \emph{Non-{Abelian} statistics of half-quantum vortices in
  $p$-wave superconductors}, Phys. Rev. Lett. \textbf{86},  268 (2001).

\bibitem{kalmeyer-87prl2095}
V.~Kalmeyer and R.~B. Laughlin, \emph{Equivalence of the
  resonating-valence-bond and fractional quantum {Hall} states}, Phys. Rev.
  Lett. \textbf{59},  2095 (1987).

\bibitem{kalmeyer-89prb11879}
---, \emph{Theory of the spin liquid state of the heisenberg antiferromagnet},
  Phys. Rev. B \textbf{39},  11879 (1989).

\bibitem{kaplan-82prl889}
T.~A. Kaplan, P.~Horsch, and P.~Fulde, \emph{Close relation between
  localized-electron magnetism and the paramagnetic wave function of completely
  itinerant electrons}, Phys. Rev. Lett. \textbf{49},  889 (1982).

\bibitem{Kauffman93}
L.~H. Kauffman, \emph{Knots and Physics} (World Scientific, Singapore, 1993).

\bibitem{kawakami92prb1005}
N.~Kawakami, \emph{Asymptotic {Bethe}-ansatz solution of multicomponent quantum
  systems with $1/r^2$ long-range interaction}, Phys. Rev.~B \textbf{46},  1005
  (1992).

\bibitem{kawakami92prb3191}
---, \emph{{SU($N$)} generalization of the {Gutzwiller--Jastrow} wave function
  and its critical properties in one dimension}, Phys. Rev.~B \textbf{46},
  3191 (1992).

\bibitem{khare05}
A.~Khare, \emph{Fractional Statistics and Quantum Theory} (World Scientific,
  New Jersey, 2005).

\bibitem{Kitaev06ap2}
A.~Kitaev, \emph{Anyons in an exactly solved model and beyond}, Ann.~of Phys.
  \textbf{321},  2 (2006).

\bibitem{kitaev02ap2}
A.~Y. Kitaev, \emph{Fault-tolerant quantum computation by anyons}, Ann. Phys.
  \textbf{303},  2 (2002).

\bibitem{kivelson-88prl2630}
S.~A. Kivelson and D.~S. Rokhsar, \emph{Quasiparticle statistics in
  time-reversal invariant states}, Phys. Rev. Lett. \textbf{61},  2630 (1988).

\bibitem{kivelson-87prb8865}
S.~A. Kivelson, D.~S. Rokhsar, and J.~P. Sethna, \emph{Topology of the
  resonating valence-bond state: Solitons and high-$t_c$ superconductivity},
  Phys. Rev. B \textbf{35},  8865 (1987).

\bibitem{kopnin-91prb9667}
N.~B. Kopnin and M.~M. Salomaa, \emph{Mutual friction in superfluid $^{3}he$:
  Effects of bound states in the vortex core}, Phys. Rev. B \textbf{44},  9667
  (1991).

\bibitem{KorepinBogoliubovIzergin93}
V.~E. Korepin, N.~M. Bogoliubov, and A.~G. Izergin, \emph{Quantum Inverse
  Scattering Method and Correlation Functions} (Cambridge University Press,
  Cambridge, 1997).

\bibitem{kuramoto-91prl1338}
Y.~Kuramoto and H.~Yokoyama, \emph{Exactly soluble supersymmetric
  {$t$}-{$J$}-type model with a long-range exchange and transfer}, Phys. Rev.
  Lett. \textbf{67},  1338 (1991).

\bibitem{landau30zp629}
L.~Landau, \emph{Diamagnetismus der {Metalle}}, Z. Phys. \textbf{64},  629
  (1930).

\bibitem{Landau1}
L.~D. Landau and E.~M. Lifshitz, \emph{Mechanics} (Butterworth-Heinemann,
  Oxford, 1982).

\bibitem{Lang85}
S.~Lang, \emph{Complex Analysis} (Springer, New York, 1985).

\bibitem{laughlin84ss163}
R.~Laughlin, \emph{Primitive and composite ground states in the fractional
  quantum {Hall} effect}, Surf.\ Sci.\ \textbf{142},  163  (1984).

\bibitem{laughlin83prl1395}
R.~B. Laughlin, \emph{Anomalous quantum {Hall} effect: {A}n incompressible
  quantum fluid with fractionally charged excitations}, Phys. Rev. Lett.
  \textbf{50},  1395 (1983).

\bibitem{laughlin-00proc}
R.~B. Laughlin, D.~Giuliano, R.~Caracciolo, and O.~L. White, \emph{Quantum
  number fractionalization in antiferromagnets}, in G.~Morandi, P.~Sodano,
  A.~Tagliacozzo, and V.~Tognetti, eds., \emph{Field Theories for
  Low-Dimensional Condensed Matter Systems} (Springer, Berlin, 2000).

\bibitem{laughlin-90prb664}
R.~B. Laughlin and Z.~Zou, \emph{Properties of the chiral-spin-liquid state},
  Phys. Rev. B \textbf{41},  664 (1990).

\bibitem{lee-07prl236807}
S.-S. Lee, S.~Ryu, C.~Nayak, and M.~P.~A. Fisher, \emph{Particle-hole symmetry
  and the $\nu{}=\frac{5}{2}$ quantum {Hall} state}, Phys. Rev. Lett.
  \textbf{99},  236807 (2007).

\bibitem{leinaas-77ncb1}
J.~M. Leinaas and J.~Myrheim, \emph{On the theory of identical particles},
  Nuovo Cimento~B \textbf{37},  1 (1977).

\bibitem{levin-07prl236806}
M.~Levin, B.~I. Halperin, and B.~Rosenow, \emph{Particle-hole symmetry and the
  {Pfaffian} state}, Phys. Rev. Lett. \textbf{99},  236806 (2007).

\bibitem{macdonald84prb3550}
A.~H. MacDonald, \emph{{Laughlin} states in higher {Landau} levels}, Phys. Rev.
  B \textbf{30},  3550 (1984).

\bibitem{marshall55prsla48}
W.~Marshall, \emph{Antiferromagnetism}, Proc. R. Soc. (London), Ser.~A
  \textbf{232},  48 (1955).

\bibitem{metha-75jmp1256}
M.~L. Mehta and G.~C. Mehta, \emph{Discrete {Coulomb} gas in one dimension:
  Correlation functions}, J. Math. Phys. \textbf{16},  1256 (1975).

\bibitem{meng-10n847}
Z.~Y. Meng, T.~C. Lang, S.~Wessel, F.~F. Assaad, and A.~Muramatsu,
  \emph{Quantum spin liquid emerging in two-dimensional correlated {Dirac}
  fermions}, Nature \textbf{464},  847 (2010).

\bibitem{metzner-87prl121}
W.~Metzner and D.~Vollhardt, \emph{Ground-state properties of correlated
  fermions: Exact analytic results for the {Gutzwiller} wave function}, Phys.
  Rev. Lett. \textbf{59},  121 (1987).

\bibitem{moessner-01prl1881}
R.~Moessner and S.~L. Sondhi, \emph{Resonating valence bond phase in the
  triangular lattice quantum dimer model}, Phys. Rev. Lett. \textbf{86},  1881
  (2001).

\bibitem{moeller08prb075319}
G.~M\"oller and S.~H. Simon, \emph{Paired composite-fermion wave functions},
  Phys. Rev. B \textbf{77},  075319 (2008).

\bibitem{moore-91npb362}
G.~Moore and N.~Read, \emph{Nonabelions in the fractional quantum {Hall}
  effect}, Nucl. Phys. B \textbf{360},  362 (1991).

\bibitem{moore09p82}
J.~E. Moore, \emph{Quasiparticles do the twist}, Physics \textbf{2},  82
  (2009).

\bibitem{morf98prl1505}
R.~H. Morf, \emph{Transition from quantum {Hall} to compressible states in the
  second {Landau} level: New light on the $\nu = 5/2$ enigma}, Phys. Rev. Lett.
  \textbf{80},  1505 (1998).

\bibitem{nayak-08rmp1083}
C.~Nayak, S.~H. Simon, A.~Stern, M.~Freedman, and S.~Das~Sarma, Rev. Mod. Phys.
  \textbf{80},  1083 (2008).

\bibitem{nayak-96npb529}
C.~Nayak and F.~Wilczek, \emph{$2n$-quasihole states realize
  $2^{n-1}$-dimensional spinor braiding statistics in paired quantum {Hall}
  states}, Nucl. Phys. B \textbf{479},  529 (1996).

\bibitem{orenstein-00s468}
J.~Orenstein and A.~J. Millis, \emph{Advances in the physics of
  high-temperature superconductivity}, Science \textbf{288},  468 (2000).

\bibitem{pan-99prl3530}
W.~Pan, J.-S. Xia, V.~Shvarts, D.~E. Adams, H.~L. Stormer, D.~C. Tsui, L.~N.
  Pfeiffer, K.~W. Baldwin, and K.~W. West, \emph{Exact quantization of the
  even-denominator fractional quantum {Hall} state at $\nu{}=5/2$ {Landau}
  level filling factor}, Phys. Rev. Lett. \textbf{83},  3530 (1999).

\bibitem{pan-08prb075307}
W.~Pan, J.~S. Xia, H.~L. Stormer, D.~C. Tsui, C.~Vicente, E.~D. Adams, N.~S.
  Sullivan, L.~N. Pfeiffer, K.~W. Baldwin, and K.~W. West, \emph{Experimental
  studies of the fractional quantum {Hall} effect in the first excited {Landau}
  level}, Phys. Rev. B \textbf{77},  075307 (2008).

\bibitem{PrangeGirvin90}
R.~Prange and S.~Girvin, eds., \emph{The Quantum Hall Effect} (Springer, New
  York, 1990), second edition.

\bibitem{radu-08s899}
I.~P. Radu, J.~B. Miller, C.~M. Marcus, M.~A. Kastner, L.~N. Pfeiffer, and
  K.~W. West, \emph{Quasi-particle properties from tunneling in the $\nu = 5/2$
  fractional quantum {Hall} state}, Science \textbf{320},  899 (2008).

\bibitem{read-00prb10267}
N.~Read and D.~Green, \emph{Paired states of fermions in two dimensions with
  breaking of parity and time-reversal symmetries and the fractional quantum
  {Hall} effect}, Phys. Rev. B \textbf{61},  10267 (2000).

\bibitem{Read-99prb8084}
N.~Read and E.~Rezayi, \emph{Beyond paired quantum {Hall} states: Parafermions
  and incompressible states in the first excited {Landau} level}, Phys. Rev. B
  \textbf{59},  8084 (1999).

\bibitem{manuscriptinpreparationSG}
B.~Scharfenberger and M.~Greiter, manuscript in preparation.

\bibitem{Schrieffer64}
J.~R. Schrieffer, \emph{Theory of {S}uperconductivity} (Benjamin/Addison
  Wesley, New York, 1964).

\bibitem{schroeter-07prl097202}
D.~F. Schroeter, E.~Kapit, R.~Thomale, and M.~Greiter, \emph{Spin {Hamiltonian}
  for which the chiral spin liquid is the exact ground state}, Phys. Rev. Lett.
  \textbf{99},  097202 (2007).

\bibitem{schwinger65proc}
J.~Schwinger, in L.~Biedenharn and H.~van Dam, eds., \emph{Quantum Theory of
  Angular Momentum} (Academic Press, New York, 1965).

\bibitem{shastry88prl639}
B.~S. Shastry, \emph{Exact solution of an {$S=\tfrac{1}{2}$} {Heisenberg}
  antiferromagnetic chain with long-ranged interactions}, Phys. Rev. Lett.
  \textbf{60},  639 (1988).

\bibitem{shastry92prl164}
---, \emph{Taking the square root of the discrete $1/r^2$ model}, Phys. Rev.
  Lett. \textbf{69},  164 (1992).

\bibitem{simon83prl2167}
B.~Simon, \emph{Holonomy, the quantum adiabatic theorem, and {Berry}'s phase},
  Phys. Rev. Lett. \textbf{51},  2167 (1983).

\bibitem{simon-07prb195306}
S.~H. Simon, E.~H. Rezayi, and N.~R. Cooper, \emph{Pseudopotentials for
  multiparticle interactions in the quantum {Hall} regime}, Phys. Rev. B
  \textbf{75},  195306 (2007).

\bibitem{simon-07prb075317}
S.~H. Simon, E.~H. Rezayi, N.~R. Cooper, and I.~Berdnikov, \emph{Construction
  of a paired wave function for spinless electrons at filling fraction
  $\nu=2/5$}, Phys. Rev. B \textbf{75},  075317 (2007).

\bibitem{stern08ap204}
A.~Stern, \emph{Anyons and the quantum {Hall} effect---a pedagogical review},
  Annals of Physics \textbf{323},  204  (2008). January Special Issue 2008.

\bibitem{stern10n187}
---, \emph{Non-{Abelian} states of matter}, Nature \textbf{464},  187 (2010).

\bibitem{stern-04prb205338}
A.~Stern, F.~von Oppen, and E.~Mariani, \emph{Geometric phases and quantum
  entanglement as building blocks for non-{Abelian} quasiparticle statistics},
  Phys. Rev. B \textbf{70},  205338 (2004).

\bibitem{storni-10prl076803}
M.~Storni, R.~H. Morf, and S.~Das~Sarma, \emph{Fractional quantum {Hall} state
  at $\nu{}=\frac{5}{2}$ and the {Moore-Read} {Pfaffian}}, Phys. Rev. Lett.
  \textbf{104},  076803 (2010).

\bibitem{sutherland71pra2019}
B.~Sutherland, \emph{Exact result for a quantum many-body problem in one
  dimension}, Phys. Rev.~A \textbf{4},  2019 (1971).

\bibitem{sutherland71jmp246}
---, \emph{Quantum many-body problem in one dimension: {G}round state},
  J.~Math. Phys. \textbf{12},  246 (1971).

\bibitem{sutherland71jmp251}
---, \emph{Quantum many-body problem in one dimension: {T}hermodynamics},
  J.~Math. Phys. \textbf{12},  251 (1971).

\bibitem{sutherland72pra1372}
---, \emph{Exact result for a quantum many-body problem in one dimension.
  {II}}, Phys. Rev.~A \textbf{5},  1372 (1972).

\bibitem{talstra95}
J.~C. Talstra, \emph{Integrability and applications of the exactly-solvable
  {Haldane--Shastry} one-dimensional quantum spin chain}, Ph.D. thesis,
  Department of Physics, Princeton University (1995).

\bibitem{talstra-95jpa2369}
J.~C. Talstra and F.~D.~M. Haldane, \emph{Integrals of motion of the
  {Haldane--Shastry} model}, J.~Phys.~A: Math. Gen. \textbf{28},  2369 (1995).

\bibitem{thomale-10prl116805}
R.~Thomale, D.~P. Arovas, and B.~A. Bernevig, \emph{Nonlocal order in gapless
  systems: Entanglement spectrum in spin chains}, Phys. Rev. Lett.
  \textbf{105},  116805 (2010).

\bibitem{thomale-09prb104406}
R.~Thomale, E.~Kapit, D.~F. Schroeter, and M.~Greiter, \emph{Parent
  {Hamiltonian} for the chiral spin liquid}, Phys. Rev. B \textbf{80},  104406
  (2009).

\bibitem{manuscriptinpreparationTRSG11}
R.~Thomale, S.~Rachel, P.~Schmitteckert, and M.~Greiter, manuscript in
  preparation.

\bibitem{thomale-10prl180502}
R.~Thomale, A.~Sterdyniak, N.~Regnault, and B.~A. Bernevig, \emph{Entanglement
  gap and a new principle of adiabatic continuity}, Phys. Rev. Lett.
  \textbf{104},  180502 (2010).

\bibitem{Tinkham96}
M.~Tinkham, \emph{Introduction to Superconductivity} (McGraw Hill, New York,
  1996).

\bibitem{trugman-85prb5280}
S.~A. Trugman and S.~Kivelson, \emph{Exact results for the fractional quantum
  {Hall} effect with general interactions}, Phys. Rev. B \textbf{31},  5280
  (1985).

\bibitem{tsui-82prl1559}
D.~C. Tsui, H.~L. Stormer, and A.~C. Gossard, \emph{Two-dimensional
  magnetotransport in the extreme quantum limit}, Phys. Rev. Lett. \textbf{48},
   1559 (1982).

\bibitem{wen-89prb11413}
X.~G. Wen, F.~Wilczek, and A.~Zee, \emph{Chiral spin states and
  superconductivity}, Phys. Rev. B \textbf{39},  11413 (1989).

\bibitem{wess-71plb95}
J.~Wess and B.~Zumino, \emph{Consequences of anomalous ward identities}, Phys.
  Lett. \textbf{37B},  95 (1971).

\bibitem{wilczek82prl1144}
F.~Wilczek, \emph{Magnetic flux, angular momentum, and statistics}, Phys. Rev.
  Lett. \textbf{48},  1144 (1982).

\bibitem{wilczek82prl957}
---, \emph{Quantum mechanics of fractional-spin particles}, Phys. Rev. Lett.
  \textbf{49},  957 (1982).

\bibitem{wilczek90}
---, \emph{Fractional statistics and anyon superconductivity} (World
  Scientific, Singapore, 1990).

\bibitem{WilczekShapere89}
F.~Wilczek and A.~Shapere, \emph{Geometric Phases in Physics} (World
  Scientific, Singapore, 1989).

\bibitem{wilczek-84prl52}
F.~Wilczek and A.~Zee, \emph{Appearance of gauge structure in simple dynamical
  systems}, Phys. Rev. Lett. \textbf{52},  2111 (1984).

\bibitem{willet-87prl1776}
R.~Willett, J.~P. Eisenstein, H.~L. St\"ormer, D.~C. Tsui, A.~C. Gossard, and
  J.~H. English, \emph{Observation of an even-denominator quantum number in the
  fractional quantum {Hall} effect}, Phys. Rev. Lett. \textbf{59},  1776
  (1987).

\bibitem{wilson62jmp1040}
K.~G. Wilson, \emph{Proof of a conjecture by {Dyson}}, J.~Math. Phys.
  \textbf{3},  1040 (1962).

\bibitem{witten84cmp455}
E.~Witten, \emph{Non-{Abelian} bosonization in two dimensions}, Commun. Math.
  Phys. \textbf{92},  455 (1984).

\bibitem{wu84prl2103}
Y.-S. Wu, \emph{General theory for quantum statistics in two dimensions}, Phys.
  Rev. Lett. \textbf{52},  2103 (1984).

\bibitem{xia-04prl176809}
J.~S. Xia, W.~Pan, C.~L. Vicente, E.~D. Adams, N.~S. Sullivan, H.~L. Stormer,
  D.~C. Tsui, L.~N. Pfeiffer, K.~W. Baldwin, and K.~W. West, \emph{Electron
  correlation in the second {Landau} level: A competition between many nearly
  degenerate quantum phases}, Phys. Rev. Lett. \textbf{93},  176809 (2004).

\bibitem{yao-07prl247203}
H.~Yao and S.~A. Kivelson, \emph{Exact chiral spin liquid with non-{Abelian}
  anyons}, Phys. Rev. Lett. \textbf{99},  247203 (2007).

\bibitem{yoshioka-83prl1219}
D.~Yoshioka, B.~I. Halperin, and P.~A. Lee, \emph{Ground state of
  two-dimensional electrons in strong magnetic fields and $\frac{1}{3}$
  quantized {Hall} effect}, Phys. Rev. Lett. \textbf{50},  1219 (1983).

\bibitem{zaanen-06np138}
J.~Zaanen, S.~Chakravarty, T.~Senthil, P.~Anderson, P.~Lee, J.~Schmalian,
  M.~Imada, D.~Pines, M.~Randeria, C.~Varma, M.~Vojta, and M.~Rice,
  \emph{Towards a complete theory of high ${T}_{\rm c}$}, Nature Physics
  \textbf{2},  138 (2006).

\bibitem{zhang-10prl166801}
C.~Zhang, T.~Knuuttila, Y.~Dai, R.~R. Du, L.~N. Pfeiffer, and K.~W. West,
  \emph{$\nu{}=5/2$ fractional quantum {Hall} effect at 10 {T}: Implications
  for the {Pfaffian} state}, Phys. Rev. Lett. \textbf{104},  166801 (2010).

\bibitem{zhang-88prb3759}
F.~C. Zhang and T.~M. Rice, \emph{Effective {H}amiltonian for the
  superconducting {Cu} oxides}, Phys. Rev. B \textbf{37},  3759 (1988).

\bibitem{zou-89prb11424}
Z.~Zou, B.~Doucot, and B.~S. Shastry, \emph{Equivalence of fractional {Hall}
  and resonating-valence-bond states on a square lattice}, Phys. Rev. B
  \textbf{39},  11424 (1989).

\end{thebibliography}

